Optimal Neighborhood Exploration for Dynamic Independent Sets

A dynamic graph algorithm is a data structure that supports edge insertions, deletions, and specific problem queries. While extensive research exists on dynamic algorithms for graph problems solvable in polynomial time, most of these algorithms have not been implemented or empirically evaluated. This work addresses the NP-complete maximum weight and cardinality independent set problems in a dynamic setting, applicable to areas like dynamic map-labeling and vehicle routing. Real-world instances can be vast, with millions of vertices and edges, making it challenging to find near-optimal solutions quickly. Exact solvers can find optimal solutions but have exponential worst-case runtimes. Conversely, heuristic algorithms use local search techniques to improve solutions by optimizing vertices. In this work, we introduce a novel local search technique called optimal neighborhood exploration. This technique creates independent subproblems that are solved to optimality, leading to improved overall solutions. Through numerous experiments, we assess the effectiveness of our approach and compare it with other state-of-the-art dynamic solvers. Our algorithm features a parameter, the subproblem size, that balances running time and solution quality. With this parameter, our configuration matches state-of-the-art performance for the cardinality independent set problem. By increasing the parameter, we significantly enhance solution quality.

==> reduction_list.tex <==


\begin{reduction}[Neighborhood Removal \cite{DBLP:conf/alenex/Lamm0SWZ19}] \label{red: neighborhood removal}
	For any $v\in V$, if $\omega(v)\geq \omega(N(v))$ then $v$ is in some MWIS of $G$. Let $G' = G[V\setminus N[v]]$ and $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$.
\end{reduction}

\begin{reduction}[Degree-One \cite{gu2021towards}]\label{red: deg1}
	Let $v$ be a degree-one vertex with the neighbor $u$ in $G$.
	\begin{itemize}
		\item Case 1: if $\omega(v) \geq \omega(u)$, $v$ must be contained in some MWIS of $G$; thus $v$ can be removed from $G$, \ie $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is the graph obtained by removing both $v$ and $u$.
		\item Case 2: if $\omega(v) < \omega(u)$, $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is the graph obtained by removing $v$ and updating the weight of $u$ to be $\omega(u) = \omega(u) - \omega(v)$. It holds that $u \in \I $ iff $u \in \I'$.
	\end{itemize}

We note that Case 1 is a special case of Reduction~\ref{red: neighborhood removal}.
\end{reduction}


\begin{reduction}[Triangle \cite{gu2021towards}]\label{red: triangle}
	This reduction is illustrated in Figure~\ref{fig: triangle_reduction}. 
	Let $v$ be a degree-two vertex with two neighbors $x$ and $y$ in $G$, where edge ${\{x,y\} \in E}$. Without loss of generality, assume ${\omega(x) \leq \omega(y)}$.
	\begin{itemize}
            \item Case 1: if $\omega(v) \geq \omega(y)$, $v$ must be contained in some MWIS of $G$. This leads to $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is obtained by removing $v$, $x$, $y$.
		\item Case 2: if $\omega(x) \leq \omega(v) < \omega(y)$, $\alpha_\omega(G) = \alpha_\omega(G')+ \omega(v)$, where $G'$ is the graph obtained by removing nodes $v$ and $x$, and updating $\omega(y)  = \omega(y) - \omega(v)$. It holds that $y \in \I$ iff $y \in \I'$.
		\item Case 3: if $\omega(v) < \omega(x)$, $\alpha_\omega(G) = \alpha_\omega(G')+ \omega(v)$, where $G'$ is the graph obtained by removing $v$, and updating $\omega(x)  = \omega(x) - \omega(v)$ as well as $\omega(y)  = \omega(y) - \omega(v)$. It holds for $z\in\{x,y\}$ that $z \in \I$ iff $z \in \I'$.
	\end{itemize}

\end{reduction}


\begin{reduction} [Extended V-Shape \cite{DBLP:conf/alenex/Lamm0SWZ19,gu2021towards}]\label{red: extended_v_shape}
	Let $v$ be a degree-two vertex with the neighbors $x$ and $y$ in $G$, where edge ${\{x,y\} \notin E}$. Without loss of generality, assume ${\omega(x) \leq \omega(y)}$.
	\begin{itemize}
		\item Case 1: \cite{DBLP:conf/alenex/Lamm0SWZ19} if $\omega(v) \geq \omega(y)$ 
		\begin{itemize} 
			\item if $\omega(v) \geq \omega(x) + \omega(y)$, $v$ must be contained in some MWIS of $G$ and this leads to $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is obtained by removing $v, x, y$. 
			\item else we fold $v,x,y$ into a vertex $v'$ with weight $\omega(v') = \omega(x) + \omega(y) - \omega(v)$ forming a new graph $G'$. Then $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$. If $v'\in \I'$ then $\{x,y\}\subset \I$, otherwise $v \in \I$.
			It holds that $\{x,y\} \subset \I$ iff $v' \in \I'$;\\
			
		\end{itemize}
		\item Case 2: \cite{gu2021towards} if ${\omega(x) \leq \omega(v) < \omega(y)}$, $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is the graph obtained by removing $v$, updating $N(x) = N(x) \cup N(y)$ and ${\omega(y) = \omega(y) - \omega(v)}$. It holds that $\forall w \in \{x,y\}$, $w \in \I$ iff ${w \in \I'}$;\\
		\item Case 3: \cite{gu2021towards} if $\omega(x) > \omega(v)$, $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$, where $G'$ is the graph obtained by updating ${\omega(x) = \omega(x) - \omega(v)}$, $\omega(y) = \omega(y) - \omega(v)$, and ${N(v) = N(x) \cup N(y)}$. It holds that $\{x,y\}\subseteq \I$ iff ${\{x,y\}\subseteq \I'}$.
	\end{itemize}
\end{reduction}

\begin{reduction}[Isolated Vertex Removal \cite{DBLP:conf/alenex/Lamm0SWZ19}] \label{red: clique} %
	Let $v\in V$ be isolated and $\omega(v)\geq \max_{u\in N(v)}\omega(u)$. Then $v$ is in some MWIS of $G$. Let $G' = G[V\setminus N[v]]$ and $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$.
\end{reduction}

\begin{reduction}[Basic Single-Edge \cite{gu2021towards}]\label{red: bse}
	Given an edge $e(u,v) \in E_G$, if $\omega(v) + \omega(N(u) \setminus N(v)) \leq\omega(u)$, it holds that $\alpha_\omega(G) = \alpha_\omega(G')$, where $G'$ is obtained by removing $v$ from $G$.
\end{reduction}

\begin{reduction}[Extended Single-Edge \cite{gu2021towards}]\label{red: ese}
	Given an edge $e(u,v) \in E_G$, if $\omega(v) \geq \omega(N(v))-\omega(u)$, it holds that $\alpha_\omega(G) = \alpha_\omega(G')$, where $G'$ is obtained by removing all vertices in $N(u) \cap N(v)$.
\end{reduction}

\begin{reduction}[Domination \cite{DBLP:conf/alenex/Lamm0SWZ19}]\label{red: dom}
	Let $u,v\in V$ be vertices such that $N[u]\supseteq N[v]$ (i.e., $u$ dominates $v$). If $\omega(u)\leq \omega(v)$, there is an MWIS in $G$ that excludes $u$ and $\alpha_\omega(G) = \alpha_\omega(G[V\setminus \{u\}])$. Therefore, $u$ can be removed from the graph.
\end{reduction}

\begin{reduction}[Twin \cite{DBLP:conf/alenex/Lamm0SWZ19}]\label{red: twin}
	Let vertices $u$ and $v$ have equal neighborhoods $N(u) = N(v) = \{p,q,r\}$, forming an independent set.
	We have two cases:
	\begin{enumerate}
		\item If $\omega(\{u,v\}) \geq \omega(\{p,q,r\})$, then $u$ and $v$ are in some MWIS of $G$. Let $G' = G[V\setminus N[\{u,v\}]]$.
		\item If $\omega(\{u,v\}) < \omega(\{p,q,r\})$, but $\omega(\{u,v\}) > \omega(\{p,q,r\}) - \min_{x\in\{p,q,r\}} \omega(x)$, then we can fold $u, v, p, q, r$ into a new vertex $v'$ with weight $\omega(v') = \omega(\{p,q,r\}) - \omega(\{u,v\})$ and call this graph $G'$. Then we construct an MWIS $\I$ of $G$ as follows: if $v'\in \I'$ then $\I = (\I'\setminus \{v'\})\cup \{p,q,r\}$, if $v'\notin \I'$ then $\I = \I' \cup \{u,v\}$.
	\end{enumerate}
	Furthermore, $\alpha_\omega(G) = \alpha_\omega(G') + \omega(\{u,v\})$.
\end{reduction}


\begin{reduction}[Simplicial Weight Transfer \cite{DBLP:conf/alenex/Lamm0SWZ19}] \label{red: clique_neigh}%
	Let $v\in V$ be isolated, and suppose that the set of simplicial vertices $S(v)\subseteq N(v)$ is such that $\forall u\in S(v)$, $\omega(v) \geq \omega(u)$. We
	\begin{enumerate}
		\item remove all $u\in N(v)$ such that $\omega(u)\leq \omega(v)$, and let the remaining neighbors be denoted by $N'(v)$,
		\item remove $v$ and $\forall x\in N'(v)$ set its new weight to $\omega'(x) = \omega(x) - \omega(v)$, and
	\end{enumerate}
	let the resulting graph be denoted by $G'$. Then $\alpha_\omega(G) = \omega(v) + \alpha_\omega(G')$ and an MWIS $\I$ of $G$ can be constructed from an MWIS $\I'$ of $G'$ as follows: if $\I' \cap N'(v) = \emptyset$ then $\I = \I'\cup\{v\}$, otherwise $\I = \I'$.
\end{reduction}

\begin{reduction}[CWIS \cite{butenko-trukhanov}]\label{red: CWIS}
Let $I_c\subseteq V$ be a critical weighted IS of $G$, \ie $\omega(\I_c) - \omega(N(\I_c)) = \max\{\omega(\I)-\omega(N(\I)) : \I \text{is an IS of G} \}$. Then $\I_c$ is in some MWIS of $G$. We set $G' = G[V\setminus N[\I_c]]$ and $\alpha_\omega(G) = \alpha_\omega(G') + \omega(\I_c)$.
\end{reduction}

\begin{reduction}[Neighborhood Folding \cite{DBLP:conf/alenex/Lamm0SWZ19}] \label{red: neighborhood folding}
Let $v \in V$, and suppose that $N(v)$ is independent. If $\omega(N(v)) > \omega(v)$, but $\omega(N(v)) - \min_{u\in N(v)}\{\omega(u)\} < \omega(v)$, then fold $v$ and $N(v)$ into a new vertex $v'$ with weight $\omega(v') = \omega(N(v)) - \omega(v)$. If $v'\in \I'$ then $\I = (\I'\setminus\{v'\}) \cup N(v)$, otherwise if $v\in \I'$ then $\I = \I' \cup \{v\}$. Furthermore, $\alpha_\omega(G) = \alpha_\omega(G') + \omega(v)$.
\end{reduction}



